Graph Coarsening via Convolution Matching for Scalable Graph Neural Network Training

Graph summarization as a preprocessing step is an effective and complementary technique for scalable graph neural network (GNN) training. In this work, we propose the Coarsening Via Convolution Matching (CONVMATCH) algorithm and a highly scalable variant, A-CONVMATCH, for creating summarized graphs that preserve the output of graph convolution. We evaluate CONVMATCH on six real-world link prediction and node classification graph datasets, and show it is efficient and preserves prediction performance while significantly reducing the graph size. Notably, CONVMATCH achieves up to 95% of the prediction performance of GNNs on node classification while trained on graphs summarized down to 1% the size of the original graph. Furthermore, on link prediction tasks, CONVMATCH consistently outperforms all baselines, achieving up to a 2x improvement.

==> figures/memoryConsumption.tex <==
\begin{figure*}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/CiteseerLPMemoryConsumption.png}
  % \caption{}
  \label{fig:CiteseerLPMemoryConsumption}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/CoraLPMemoryConsumption.png}
  % \caption{}
  \label{fig:CoraLPMemoryConsumption}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/OGBLCollabMemoryConsumption.png}
  % \caption{}
  \label{fig:OGBLCollabLPMemoryConsumption}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/OGBLCitation2MemoryConsumption.png}
  % \caption{}
  \label{fig:OGBLCitaion2LPMemoryConsumption}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/CiteseerNCMemoryConsumption.png}
  % \caption{}
  \label{fig:CiteseerNCMemoryConsumption}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/CoraNCMemoryConsumption.png}
  % \caption{}
  \label{fig:CoraNCMemoryConsumption}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/OGBNArxivMemoryConsumption.png}
  % \caption{}
  \label{fig:OGBNArxivMemoryConsumption}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/OGBNProductsMemoryConsumption.png}
  % \caption{}
  \label{fig:OGBNProductsMemoryConsumption}
\end{subfigure}
\caption{Plots of GPU memory consumption during training with graphs at multiple coarsening ratios for each dataset.}
\label{fig:memoryConsumption}
\end{figure*}

==> figures/trainingTime.tex <==
\begin{figure*}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/CiteseerLPTrainingTime.png}
  % \caption{}
  \label{fig:CiteseerLPTrainingTime}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/CoraLPTrainingTime.png}
  % \caption{}
  \label{fig:CoraLPTrainingTime}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/OGBLCollabTrainingTime.png}
  % \caption{}
  \label{fig:OGBLCollabTrainingTime}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/OGBLCitation2TrainingTime.png}
  % \caption{}
  \label{fig:OGBLCitation2TrainingTime}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/CiteseerNCTrainingTime.png}
  % \caption{}
  \label{fig:CiteseerNCTrainingTime}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/CoraNCTrainingTime.png}
  % \caption{}
  \label{fig:CoraNCTrainingTime}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/OGBNArxivTrainingTime.png}
  % \caption{}
  \label{fig:OGBNArxivTrainingTime}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/OGBNProductsTrainingTime.png}
  % \caption{}
  \label{fig:OGBNProductsTrainingTime}
\end{subfigure}
\caption{Plots of the average time required to complete all training epochs for each dataset at varying coarsening ratios.}
\label{fig:trainingTime}
\end{figure*}

==> sections/tables/link_prediction_graph_summarization_times.tex <==
% {\small
\begin{table}[h]
    \centering
    \begin{tabular}{cc|ccc}
    \toprule
        && \multicolumn{3}{c}{\textbf{Coarsening Ratio (r)}} \\
         \cline{3-5}
         & \textbf{Summarizer}  & $0.1\%$ & $1\%$ & $10\%$ \\
    \midrule
        \multirow{5}{*}{\rotatebox{90}{Citeseer}} 
        & GCond & $ - $ & $ 3,281 \pm 23.84 $  & $ 23,996 \pm 400.82 $ \\
        & DosCond & $ - $ & $ 142.21 \pm 1.85 $  & $ 682.83 \pm 9.85 $ \\
        & VN & $ - $ & $ 8.26 \pm 1.23 $  & $ 8.30 \pm 1.58 $ \\
        \cline{2-5}
        & \shortname{}  & $ - $ & $ - \pm - $  & $ - \pm - $ \\
        & A-\shortname{}  & $ - $ & $ 184.58 \pm 7.59 $  & $ 166.33 \pm 7.38 $ \\
    \hline
        \multirow{5}{*}{\rotatebox{90}{Cora}} 
        & GCond & $ - $ & $ 4,056 \pm 40.89 $  & $ - \pm - $ \\
        & DosCond & $ - $ & $ 215.36 \pm 2.84 $  & $ 695.55 \pm 4.26 $ \\
        & VN & $ - $ & $ \mathbf{6.05 \pm 0.64} $  & $ \mathbf{6.05 \pm 0.71} $ \\
        \cline{2-5}
        & \shortname{}  & $ - $ & $ - \pm - $ & $ - \pm - $ \\
        & A-\shortname{}  & $ - $ & $ 106.07 \pm 2.80 $  & $ 96.93 \pm 2.72 $ \\
    \hline
        \multirow{4}{*}{\rotatebox{90}{OGBLCol}}
        & GCond & $ - \pm - $ & OOM  & OOM \\
        & DosCond & $ 1,339 \pm 8.97 $ & OOM  & OOM \\
        & VN & $ 706.09 \pm 193.19 $ & $ 646.86 \pm 25.89 $ & $ 594.64 \pm 39.75 $ \\
        \cline{2-5}
        & A-\shortname{}  & $ \mathbf{224.07 \pm 5.01} $ & $ \mathbf{205.53 \pm 5.31} $  & $ \mathbf{177.54 \pm 5.18} $ \\
    \hline
        \multirow{4}{*}{\rotatebox{90}{OGBLCit2}}
        & GCond & OOM & OOM  & $ - $ \\
        & DosCond & OOM & OOM  & $ - $ \\
        & VN & $ - \pm - $ & $ - \pm - $  & $ - $ \\
        \cline{2-5}
        & A-\shortname{}  & $ 7,651 \pm 277 $ & $ 6,845 \pm 279 $  & $ - $ \\
    \bottomrule
    \end{tabular}
    \caption{Link Prediction Graph Summarization Times in Seconds at Varying Coarsening Levels}
    \label{tab:link_prediction_summarization_time}
\end{table}
% }%


==> sections/tables/link_prediction_performance.tex <==
% \begin{table}[h]
%     \centering
%     \caption{Link Prediction Performance at Varying Coarsening Levels. The top three performing scores are highlighted as: \colorbox{orange!50}{First}, \colorbox{orange!25}{Second}, \colorbox{orange!12}{Third}. Either \shortname{} or A-\shortname{} is the best-performing method for every dataset and coarsening ratio.}
%     \begin{tabular}{cc||cccc}
%     \toprule
%          & & \multicolumn{4}{c}{\textbf{Coarsening Ratio (r)}} \\
%          \cline{3-6}
%          & \textbf{Summarizer}  & $0.1\%$ & $1\%$ & $10\%$ & $100\%$ \\
%     \midrule
%     \midrule
%         \multirow{6}{*}{\rotatebox{90}{Citeseer}}
%         & RS & $ - $ & $ 67.41 \pm 1.26 $ & $ 69.11 \pm 2.09 $ & \multirow{6}{*}{\rotatebox{90}{$ \mathbf{91.57 \pm 0.55} $}} \\
%         & GCond & $ - $ & $ 65.01 \pm 1.09 $ &  $ 72.65 \pm 6.78$ & \\
%         & DosCond & $ - $ & $ 63.54 \pm 6.36 $ &  $ 53.06 \pm 12.28 $ & \\
%         & VN & $ - $ & \cellcolor{orange!12} $ 80.26 \pm 4.51 $ & \cellcolor{orange!25} $ 88.55 \pm 0.77 $ & \\
%         \cline{2-5}
%         & \shortname{}  & $ - $ & \cellcolor{orange!50} $ \mathbf{87.72 \pm 1.38} $ & \cellcolor{orange!50} $ \mathbf{90.43 \pm 0.49} $ & \\
%         & A-\shortname{} & $ - $ & \cellcolor{orange!25} $ 87.68 \pm 1.24 $ & \cellcolor{orange!12} $ 88.41 \pm 0.97 $ &  \\
%     \hline
%     \hline
%         \multirow{6}{*}{\rotatebox{90}{Cora}} 
%         & RS & $ - $ & $ 70.91 \pm 3.67 $ &  $ 72.84 \pm 2.15 $ & \multirow{5}{*}{\rotatebox{90}{$ \mathbf{85.04 \pm 0.68} $}} \\
%         & GCond & $ - $ & $ 67.08 \pm 0.64 $ &  $ 66.19 \pm 0.39 $ & \\
%         & DosCond & $ - $ & \cellcolor{orange!12} $ 71.60 \pm 0.35 $ &  $ 60.21 \pm 0.52 $ & \\
%         & VN & $ - $ & \cellcolor{orange!25} $ 75.19 \pm 3.01 $ & \cellcolor{orange!12} $ 81.81 \pm 2.06 $ & \\
%         \cline{2-5}
%         & \shortname{}  & $ - $ & $ 66.33 \pm 2.35 $ & \cellcolor{orange!50} $ \mathbf{83.51 \pm 1.01} $ & \\
%         & A-\shortname{} & $ - $ & \cellcolor{orange!50} $ \mathbf{78.63 \pm 1.55} $ & \cellcolor{orange!25} $ 83.30 \pm 1.45 $ & \\
%     \hline
%     \hline
%         \multirow{5}{*}{\rotatebox{90}{OGBLCol}}
%         & RS & \cellcolor{orange!12} $ 7.22 \pm 0.97 $ & \cellcolor{orange!25} $ 11.41 \pm 0.35 $ & \cellcolor{orange!12} $ 15.80 \pm 3.11 $ & \multirow{5}{*}{\rotatebox{90}{$ \mathbf{ 44.08 \pm 0.94 } $}} \\
%         & GCond & \cellcolor{orange!25} $ 7.61 \pm 0.41  $ & OOM & OOM & \\
%         & DosCond & $ 1.15 \pm 0.88 $ & OOM & OOM & \\
%         & VN & $ 6.60 \pm 1.47 $ & \cellcolor{orange!12} $ 5.45 \pm 1.95 $ & \cellcolor{orange!25} $ 24.33 \pm 1.61 $ & \\
%         \cline{2-5}
%         & A-\shortname{}  & \cellcolor{orange!50} $ \mathbf{9.14 \pm 2.07} $ & \cellcolor{orange!50} $ \mathbf{26.25 \pm 1.84} $ & \cellcolor{orange!50} $ \mathbf{35.94 \pm 1.86} $ & \\
%     \hline
%     \hline
%         \multirow{5}{*}{\rotatebox{90}{OGBLCit2}}
%         & RS & \cellcolor{orange!12} $ 9.86 \pm 0.01 $ & \cellcolor{orange!12} $ 9.87 \pm 0.01 $ & $ - $ & \multirow{5}{*}{\rotatebox{90}{$ \mathbf{ 84.74 \pm 0.00 } $}} \\
%         & GCond & OOM & OOM & $ - $ & \\
%         & DosCond & OOM & OOM & $ - $ & \\
%         & VN & \cellcolor{orange!25} $ 10.43 \pm 2.71 $ & \cellcolor{orange!25} $ 38.95 \pm 4.83 $ &  $ - $ & \\
%         \cline{2-5}
%         & A-\shortname{}  & \cellcolor{orange!50} $ \mathbf{30.42 \pm 0.63} $ & \cellcolor{orange!50} $ \mathbf{60.34 \pm 1.15} $ &  $ - $ & \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:link_prediction_performance}
% \end{table}

\begin{table}[h]
    \centering
    \caption{Link Prediction Performance at Varying Coarsening Levels. The top three performing scores are highlighted as: \colorbox{orange!50}{First}, \colorbox{orange!25}{Second}, \colorbox{orange!12}{Third}. 
    Either \shortname{} or A-\shortname{} is the best-performing method for every dataset and coarsening ratio.}
    \scalebox{0.8}{
    \begin{tabular}{cc||cccc|cc}
    \toprule
         & & \multicolumn{6}{c}{\textbf{Sumarizer}} \\
         \cline{3-8}
         & \textbf{Ratio} & RS & GCond & DosCond & VN & \shortname{} & A-\shortname{} \\
    \midrule
    \midrule
        \multirow{3}{*}{\rotatebox{90}{Citeseer}}
        & $1\%$ & $ 67.41 \pm 1.26 $ & $ 65.01 \pm 1.09 $ & $ 63.54 \pm 6.36 $ & \cellcolor{orange!12} $ 80.26 \pm 4.51 $ & \cellcolor{orange!50} $ \mathbf{87.72 \pm 1.38} $ & \cellcolor{orange!25} $ 87.68 \pm 1.24 $ \\
        & $10\%$ & $ 69.11 \pm 2.09 $ & $ 72.65 \pm 6.78$ & $ 53.06 \pm 12.28 $ & \cellcolor{orange!25} $ 88.55 \pm 0.77 $ & \cellcolor{orange!50} $ \mathbf{90.43 \pm 0.49} $ & \cellcolor{orange!12} $ 88.41 \pm 0.97 $ \\
    \cline{3-8}
        & $100\%$ & \multicolumn{6}{c}{$ \mathbf{91.57 \pm 0.55} $} \\
    \hline
    \hline
    \multirow{3}{*}{\rotatebox{90}{Cora}}
        & $1\%$ & $ 70.91 \pm 3.67 $ & $ 67.08 \pm 0.64 $ & \cellcolor{orange!12} $ 71.60 \pm 0.35 $ & \cellcolor{orange!25} $ 75.19 \pm 3.01 $ & $ 66.33 \pm 2.35 $ & \cellcolor{orange!50} $ \mathbf{78.63 \pm 1.55} $ \\
        & $10\%$ & $ 72.84 \pm 2.15 $ & $ 66.19 \pm 0.39 $ & $ 60.21 \pm 0.52 $ & \cellcolor{orange!12} $ 81.81 \pm 2.06 $ & \cellcolor{orange!50} $ \mathbf{83.51 \pm 1.01} $ & \cellcolor{orange!25} $ 83.30 \pm 1.45 $ \\
    \cline{3-8}
        & $100\%$ & \multicolumn{6}{c}{$ \mathbf{85.04 \pm 0.68} $} \\
    \hline
    \hline
    \multirow{4}{*}{\rotatebox{90}{Coll}}
        & $.1\%$ & \cellcolor{orange!12} $ 7.22 \pm 0.97 $ & \cellcolor{orange!25} $ 7.61 \pm 0.41  $ & $ 1.15 \pm 0.88 $ & $ 6.60 \pm 1.47 $ & - & \cellcolor{orange!50} $ \mathbf{9.14 \pm 2.07} $ \\
        & $1\%$ & \cellcolor{orange!25} $ 11.41 \pm 0.35 $ & OOM & OOM & \cellcolor{orange!12} $ 5.45 \pm 1.95 $ & - & \cellcolor{orange!50} $ \mathbf{26.25 \pm 1.84} $ \\
        & $10\%$ & \cellcolor{orange!12} $ 15.80 \pm 3.11 $ & OOM & OOM & \cellcolor{orange!25} $ 24.33 \pm 1.61 $ & - & \cellcolor{orange!50} $ \mathbf{35.94 \pm 1.86} $ \\
    \cline{3-8}
        & $100\%$ & \multicolumn{6}{c}{$ \mathbf{44.08 \pm 0.94} $} \\
    \hline
    \hline
    \multirow{3}{*}{\rotatebox{90}{Cit2}}
        & $.1\%$ & \cellcolor{orange!12} $ 9.86 \pm 0.01 $ & OOM & OOM & \cellcolor{orange!25} $ 10.43 \pm 2.71 $ & - & \cellcolor{orange!50} $ \mathbf{30.42 \pm 0.63} $ \\
        & $1\%$ & \cellcolor{orange!12} $ 9.87 \pm 0.01 $ & OOM & OOM & \cellcolor{orange!25} $ 38.95 \pm 4.83 $ & - & \cellcolor{orange!50} $ \mathbf{60.34 \pm 1.15} $ \\
    \cline{3-8}
        & $100\%$ & \multicolumn{6}{c}{$ \mathbf{84.74 \pm 0.00} $} \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:link_prediction_performance}
\end{table}


==> sections/tables/link_prediction_training_times.tex <==
{\small
\begin{table}[h]
    \centering
    \begin{tabular}{cc||cccc}
    \toprule
         & & \multicolumn{4}{c}{\textbf{Coarsening Ratio (r)}} \\
         \cline{3-6}
         & \textbf{Summarizer}  & $0.1\%$ & $1\%$ & $10\%$ & $100\%$ \\
    \midrule
    \midrule
        \multirow{6}{*}{\rotatebox{90}{Citeseer}}
        & RS & $ \mathbf{65.11 \pm 3.56} $ & $ \mathbf{69.83 \pm 2.72} $ & $ \mathbf{70.98 \pm 3.19} $ & \multirow{6}{*}{\rotatebox{90}{$ 124 \pm 1 $}}  \\
        & GCond & $ - \pm - $ & $ - \pm - $ & $- \pm -$ & \\
        & DosCond & $ - \pm - $ & $ - \pm - $ & $- \pm -$ & \\
        & VN & $ 69.71 \pm 2.93 $ & $ 75.35 \pm 0.19 $ & $ 77.02 \pm 2.53 $ & \\\cline{2-5}
        & \shortname{} & $ 74.34 \pm 0.32 $ & $ 75.79 \pm 1.04 $ & $ 80.01 \pm 2.15 $ & \\
        & A-\shortname{} & $ 75.82 \pm 0.77 $ & $ 73.88 \pm 0.04 $ & $ 73.02 \pm 0.90 $ & \\
    \hline
        \multirow{6}{*}{\rotatebox{90}{Cora}}
        & RS & $ \mathbf{54.33 \pm 1.43} $ & $ \mathbf{63.43 \pm 2.55} $ & $ \mathbf{61.68 \pm 0.75} $ & \multirow{6}{*}{\rotatebox{90}{$ 153 \pm 1 $}}  \\
        & GCond & $ - \pm - $ & $ - \pm - $ & $- \pm -$ & \\\
        & DosCond & $ - \pm - $ & $ - \pm - $ & $- \pm -$ & \\\
        & VN & $ 62.43 \pm 1.52 $ & $ 65.19 \pm 1.27 $ & $ 64.45 \pm 0.90 $ & \\\cline{2-5}
        & \shortname{} & $ 65.32 \pm 1.39 $ & $ 97.63 \pm 4.56 $ & $ 152 \pm 2 $ & \\
        & A-\shortname{} & $ 63.34 \pm 1.08 $ & $ 92.53 \pm 3.07 $ & $ 150 \pm 1 $ & \\
    \hline
        \multirow{5}{*}{\rotatebox{90}{OGBLCol}} 
        & RS & $ 1,224\pm 21 $ & $ \mathbf{1,266 \pm 12} $ & $ \mathbf{1,426 \pm 9} $ & \multirow{5}{*}{\rotatebox{90}{$ 6,386 \pm 30 $}} \\
        & GCond & $ - \pm - $ & $ - \pm - $ & $- \pm -$ & \\
        & DosCond & $ - \pm - $ & $ - \pm - $ & $- \pm -$ & \\
        & VN & $ 1,271 \pm 21 $ & $ 1,406 \pm 7 $ & $ 1,692 \pm 10 $ & \\\cline{2-5}
        & A-\shortname{} & $ \mathbf{1,214 \pm 9} $ & $ 2,830 \pm 20 $ & $ 4,171 \pm 48 $ & \\
    \hline
        \multirow{5}{*}{\rotatebox{90}{OGBLCit2}} 
        & RS & $ \mathbf{1,665 \pm -} $ & $ \mathbf{1,737 \pm -} $ & $ - \pm - $ & \multirow{5}{*}{\rotatebox{90}{$ 65,758 \pm - $}}  \\
        & GCond & $ - \pm - $ & $ - \pm - $ & $- \pm -$ & \\
        & DosCond & $ - \pm - $ & $ - \pm - $ & $- \pm -$ & \\
        & VN & $ 2,167 \pm - $ & $ 9,861 \pm - $ & $- \pm -$ & \\\cline{2-5}
        & A-\shortname{} & $ 2,856 \pm - $ & $ 18,461 \pm - $ & $- \pm -$ & \\
    \hline
    \end{tabular}
    \caption{Link Prediction Training Times in Seconds at Varying Coarsening Levels}
    \label{tab:my_label}
\end{table}
}%

==> sections/tables/merge_batch_ablation_node_classification.tex <==
{\small
\begin{table}[h]
    \centering
    \caption{Graph summarization time in seconds and node classification accuracy at varying merge batch sizes and a coarsening ratio $r=1.0\%$.
    There is a large improvement in time when the batch size is increased without much sacrifice in prediction performance.
    }
    \begin{tabular}{cc|c|cc}
    \toprule
        \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Batch Size}} & \multirow{2}{*}{\textbf{Time (sec)}} & \multicolumn{2}{c}{\textbf{Accuracy}} \\
        &&& Valid. & Test.\\
    \midrule
        \multirow{3}{*}{Citeseer} 
        & $1$ & $ 198.84 $ & $ 66.92 $ & $ 66.08 $ \\
        & $10$ & $ 36.78 $ & $ 72.40 $ & $ 68.90 $ \\
        & $100$ & $ 8.03 $ & $ 65.20 $ & $ 62.30 $ \\
    \hline
        \multirow{3}{*}{Cora} 
        & $1$ & $ 101.74 $ & $ 74.40 $ & $ 74.70 $ \\
        & $10$ & $ 27.16 $ & $ 70.20 $ & $ 72.30 $ \\
        & $100$ & $ 4.89 $ & $ 71.40 $ & $ 71.20 $ \\
    \hline
    \multirow{3}{*}{OGBNArxiv} 
        & $100$ & $ 624.91 $ & $ 63.94 $ & $ 63.46 $ \\
        & $1,000$ & $ 194.73 $ & $ 62.25 $ & $ 61.07 $ \\
        & $10,000$ & $ 149.91 $ & $ 64.05 $ & $ 64.12 $ \\
    \hline
        \multirow{3}{*}{OGBNProd} 
        & $10,000$ & $ 11,285 $ & $ 85.95 $ & $ 68.57 $ \\
        & $100,000$ & $ 6,729 $ & $ 86.18 $ & $ 68.20 $ \\
    \bottomrule
    \end{tabular}
    \label{tab:merge_batch_ablation_node_classification}
\end{table}
}%

% Just time
% {\small
% \begin{table}[h]
%     \centering
%     \begin{tabular}{cc|ccc}
%     \toprule
%         & & \multicolumn{3}{c}{\textbf{Coarsening Ratio}} \\
%         \cline{3-5}
%         \multirow{1}{*}{\textbf{Dataset}} & \multirow{1}{*}{\textbf{Batch Size}} & \multicolumn{1}{c}{$\mathbf{r}=0.1\%$} & \multicolumn{1}{c}{$\mathbf{r}=1\%$} & \multicolumn{1}{c}{$\mathbf{r}=10\%$} \\
%     \midrule
%         \multirow{3}{*}{Citeseer} 
%         & $1$ & $ - \pm - $ & $ 173.70 \pm 4.96 $ & $162.27 \pm 4.92$ \\
%         & $10$ & $ - \pm - $ & $ 34.28 \pm 0.78 $ & $31.93 \pm 0.85$ \\
%         & $100$ & $ - \pm - $ & $ \mathbf{12.55 \pm 0.43} $ & $ \mathbf{11.59 \pm 0.35} $ \\
%     \hline
%         \multirow{3}{*}{Cora} 
%         & $1$ & $ - \pm - $ & $ 99.41 \pm 1.25 $ & $ 91.19 \pm 1.18 $ \\
%         & $10$ & $ - \pm - $ & $ 21.19 \pm 0.6 $ & $ 19.42 \pm 0.55 $ \\
%         & $100$ & $ - \pm - $ & $ \mathbf{5.51 \pm 0.06} $ & $ \mathbf{4.97 \pm 0.07} $ \\
%     \hline
%     \multirow{3}{*}{OGBNArxiv} 
%         & $100$ & $ - \pm - $ & $ 23,491 \pm 931 $ & $ 24,067 \pm 910 $ \\
%         & $1000$ & $ - \pm - $ & $ 1,539 \pm 135 $ & $ 1,193 \pm 121 $ \\
%         & $10,000$ & $ - \pm - $ & $ \mathbf{698 \pm 73} $ & $ \mathbf{236 \pm 24} $ \\
%     \hline
%         \multirow{3}{*}{OGBLCol} 
%         & $100$ & $ - \pm - $ & $ 23,491 \pm 931 $ & $ 24,067 \pm 910 $ \\
%         & $1000$ & $ - \pm - $ & $ 1,539 \pm 135 $ & $ 1,193 \pm 121 $ \\
%         & $10,000$ & $ - \pm - $ & $ \mathbf{698 \pm 73} $ & $ \mathbf{236 \pm 24} $ \\
%     \hline
%         \multirow{2}{*}{OGBLCit2} 
%         & $10,000$ & $ - \pm - $ & $ 9,997 \pm - $ & $ - \pm - $ \\
%         & $100,000$ & $ - \pm - $ & $ \mathbf{6,682 \pm -} $ & $ - \pm - $ \\
%     \hline
%         \multirow{2}{*}{OGBNProd} 
%         & $10,000$ & $ - \pm - $ & $ - \pm - $ & $ - \pm - $ \\
%         & $100,000$ & $ - \pm - $ & $ - \pm - $ & $ - \pm - $ \\
%     \bottomrule
%     \end{tabular}
%     \caption{Graph Summarization Time in Seconds at Varying Merge Batch Sizes and Coarsening Levels}
%     \label{tab:my_label}
% \end{table}
% }%

==> sections/tables/node_classification_accuracy.tex <==
{\footnotesize
\begin{table}[h]
    \centering
    \caption{Node Classification Accuracy at Varying Coarsening Levels. The top three performing scores are highlighted as: \colorbox{orange!50}{First}, \colorbox{orange!25}{Second}, \colorbox{orange!12}{Third}. Either \shortname{} or A-\shortname{} is among the top-3 best-performing methods for every dataset and coarsening ratio.}
    \begin{tabular}{cc||cccc}
    \toprule
         & & \multicolumn{4}{c}{\textbf{Coarsening Ratio (r)}} \\
         \cline{3-6}
         & \textbf{Summarizer}  & $0.1\%$ & $1\%$ & $10\%$ & $100\%$ \\
    \midrule
    \midrule
        \multirow{8}{*}{\rotatebox{90}{Citeseer}}
        & RS & $ - $ & $ 19.22 \pm 6.85 $ &  $ 28.00 \pm 9.15 $ & \multirow{8}{*}{\rotatebox{90}{$ \mathbf{71.40 \pm 0.35} $}} \\
        & KCenter & $ - $ & $ 59.02 \pm 2.25 $ &  $ 54.70 \pm 3.62 $ & \\
        & Herding & $ - $ & $ 62.80 \pm 1.33 $ &  $ 53.5 \pm 1.68 $ & \\
        & GCond & $ - $ & \cellcolor{orange!25} $ 68.22 \pm 2.08 $ & \cellcolor{orange!50} $ \mathbf{70.10 \pm 3.43} $ & \\
        & DosCond & $ - $ & \cellcolor{orange!50} $ \mathbf{71.36 \pm 1.27} $ & \cellcolor{orange!25} $ 68.76 \pm 0.97 $ & \\
        & VN & $ - $ & $ 35.92 \pm 3.76 $ &  $ 53.88 \pm 7.36 $ & \\
        \cline{2-5}
        & \shortname{}  & $ - $ & $ 65.40 \pm 4.12 $ & \cellcolor{orange!12} $ 69.84 \pm 1.58 $ & \\
        & A-\shortname{}  & $ - $ & \cellcolor{orange!12} $ 67.68 \pm 2.87 $ & $ 68.46 \pm 1.61 $ & \\
    \hline
    \hline
        \multirow{8}{*}{\rotatebox{90}{Cora}} 
        & RS & $ - $ & $ 18.76 \pm 9.67 $ & $ 27.52 \pm 9.89 $ & \multirow{8}{*}{\rotatebox{90}{$ \mathbf{ 81.02 \pm 0.19 }$}} \\
        & KCenter & $ - $ & $ 59.92 \pm 1.67 $ &  $ 56.12 \pm 7.46 $ & \\
        & Herding & $ - $ & $ 63.74 \pm 2.24 $ &  $ 64.10 \pm 2.12 $ & \\
        & GCond & $ - $ & \cellcolor{orange!25} $ 77.44 \pm 1.90 $ & \cellcolor{orange!25} $ 80.02 \pm 0.92 $ & \\
        & DosCond & $ - $ & \cellcolor{orange!50} $ 78.40 \pm 0.83 $ & $ 78.64 \pm 1.87 $ & \\
        & VN & $ - $ & $ 31.96 \pm 11.02 $ &  $ 59.22 \pm 4.90 $ & \\
        \cline{2-5}
        & \shortname{}  & $ - $ & \cellcolor{orange!12} $ 72.60 \pm 3.11 $ & \cellcolor{orange!12} $ 79.82 \pm 0.60 $ & \\
        & A-\shortname{}  & $ - $ & $ 72.30 \pm 2.90 $ & \cellcolor{orange!50} $ 80.12 \pm 1.09 $ & \\
    \hline
    \hline
        \multirow{7}{*}{\rotatebox{90}{OGBNArxiv}}
        & RS & $ 42.45 \pm 3.62 $ & $ 59.97 \pm 1.58 $ &  $ 67.50 \pm 0.63 $ & \multirow{7}{*}{\rotatebox{90}{$ \mathbf{72.14 \pm 0.18} $}} \\
        & KCenter & \cellcolor{orange!12} $ 49.79 \pm 2.87 $ & \cellcolor{orange!25} $ 61.99 \pm 1.24 $ & \cellcolor{orange!50} $ \mathbf{68.25 \pm 0.25} $ & \\
        & Herding & \cellcolor{orange!50} $ \mathbf{58.79 \pm 0.90} $ & \cellcolor{orange!12} $ 61.42 \pm 1.34 $ & \cellcolor{orange!25} $ 67.75 \pm 0.58 $ & \\
        & GCond & $ 48.10 \pm 3.27 $ & OOM & OOM & \\
        & DosCond & $ 21.69 \pm 4.30 $ & OOM & OOM & \\
        & VN & $ 28.90 \pm 5.79 $ & $ 53.61 \pm 2.76 $ &  $ 67.12 \pm 1.26 $ & \\
        \cline{2-5}
        & A-\shortname{}  & \cellcolor{orange!25} $ 54.82 \pm 2.67 $ & \cellcolor{orange!50} $ \mathbf{64.08 \pm 0.39} $ & \cellcolor{orange!12} $ 67.51 \pm 0.47 $ & \\
    \hline
    \hline
        \multirow{7}{*}{\rotatebox{90}{OGBNProd}}
        & RS & $ 48.20 \pm 1.57 $ & $ 66.57 \pm 1.47 $ &  $ - $ & \multirow{7}{*}{\rotatebox{90}{$ \mathbf{ 75.64 \pm 0.00 }^*$}} \\
        & KCenter & \cellcolor{orange!12} $ 60.88 \pm 1.31 $ & \cellcolor{orange!25} $ 69.66 \pm 0.31 $ &  $ - $ & \\
        & Herding & \cellcolor{orange!50} $ \mathbf{66.14 \pm 0.71} $ & \cellcolor{orange!50} $ \mathbf{71.79 \pm 0.45} $ &  $  - $ & \\
        & GCond & OOM & OOM & $ - $ & \\
        & DosCond & OOM & OOM & $ - $ & \\
        & VN & TIMEOUT & TIMEOUT &  $ - $ & \\
        \cline{2-5}
        & A-\shortname{}  & \cellcolor{orange!25} $ 62.36 \pm 0.84 $ & \cellcolor{orange!12} $ 68.20 \pm 0.36 $ &  $ - $ & \\
    \bottomrule
    \end{tabular}
    \label{tab:node_classification_accuracy}
\end{table}
}%

% 0.01, 0.05, 0.1, 0.3, 1.0
% {\small
% \begin{table*}[h]
%     \centering
%     \begin{tabular}{cc|ccccc}
%     \hline
%         \textbf{Dataset} & \textbf{Summarizer} & $\mathbf{r}=0.01$ & $\mathbf{r}=0.05$ & $\mathbf{r}=0.1$ & $\mathbf{r}=0.3$ & $\mathbf{r}=1.0$ \\
%     \midrule
%         \multirow{8}{*}{Citeseer} 
%         & RS & $ - \pm - $ & $- \pm -$ & $ - \pm - $ & $ - \pm - $ & \multirow{8}{*}{$ \mathbf{72.43 \pm 0.77} $} \\
%         & KCenter & $ 58.38 \pm 0.93 $ & $ 44.95 \pm 3.09 $ & $ 52.70 \pm 0.67 $ & $ 60.87 \pm 1.16 $ & \\
%         & Herding & $ 59.98 \pm 1.64 $ & $ 41.90 \pm 2.84 $ & $ 52.00 \pm 1.83 $ & $ 66.08 \pm 1.90 $ & \\
%         & GCond & $ 63.37 \pm 4.19 $ & $ \mathbf{71.67 \pm 0.40} $ & $ \mathbf{71.97 \pm 0.84} $ & $ - \pm - $ \\
%         & DosCond & $ \mathbf{68.57 \pm 5.93} $ & $ 61.25 \pm 1.87 $ & $ 66.97 \pm 1.16 $ & $ - \pm - $ \\
%         & VN & $ 49.23 \pm 2.65 $ & $ 64.98 \pm 4.01 $ & $ 66.78 \pm 2.78 $ & $ 69.98 \pm 1.14 $ & \\
%         \cline{2-6}
%         & ConvMatch  & $ - \pm - $ & $- \pm -$ & $ - \pm - $ & $ - \pm - $ & \\
%         & A-ConvMatch  & $ 55.48 \pm 5.9 $ & $ 67.13 \pm 2.87 $ & $ 70.63 \pm 3.02 $ & $ 71.58 \pm 0.95 $ & \\
%     \hline
%         \multirow{8}{*}{Cora} 
%         & RS & $ - \pm - $ & $- \pm -$ & $ - \pm - $ & $ - \pm - $ & \multirow{8}{*}{$ \mathbf{78.55 \pm 0.64} $} \\
%         & KCenter & $ 47.65 \pm 2.05 $ & $ 77.65 \pm 1.06 $ & $ 44.95 \pm 2.47 $ & $ 62.15 \pm 4.60 $ & \\
%         & Herding & $ 56.65 \pm 1.91 $ & $ 76.45 \pm 0.64 $ & $ 56.25 \pm 0.21 $ & $ 68.60 \pm 2.69 $ & \\
%         & GCond & $ \mathbf{75.10 \pm -} $ & $ \mathbf{79.10 \pm -} $ & $ - \pm - $ & $ - \pm - $ \\
%         & DosCond & $ 62.25 \pm 14.78 $ & $ 69.20 \pm - $ & $ - \pm - $ & $ - \pm - $ \\
%         & VN & $ 38.75 \pm 16.33 $ & $ 63.70 \pm 3.39 $ & $ 70.00 \pm 2.69 $ & $ 78.10 \pm 0.99 $ & \\
%         \cline{2-6}
%         & ConvMatch  & $ - \pm - $ & $- \pm -$ & $ - \pm - $ & $ - \pm - $ & \\
%         & A-ConvMatch  & $ 73.90 \pm 4.40 $ & $ 76.50 \pm 1.56 $ & $ 79.47 \pm 1.57 $ & $ 80.35 \pm 0.92 $ & \\
%     \hline
%         \multirow{7}{*}{OGBNArxiv} 
%         & RS & $ 58.40 \pm 2.11 $ & $ 62.24 \pm 1.35 $ & $ 64.75 \pm 0.58 $ & $ 66.41 \pm 0.40 $ & \multirow{7}{*}{$ \mathbf{68.96 \pm 0.09} $} \\
%         & KCenter & $ 44.92 \pm 1.10 $ & $ 50.84 \pm 1.88 $ & $ 62.48 \pm 0.96 $ & $ 66.61 \pm 0.51 $ & \\
%         & Herding & $ \mathbf{64.16 \pm 0.40} $ & $ \mathbf{64.98 \pm 0.35} $ & $ \mathbf{65.07 \pm 0.33} $ & $ \mathbf{67.12 \pm 0.20} $ & \\
%         & GCond & OOM & OOM & OOM & OOM \\
%         & DosCond & OOM & OOM & OOM & OOM \\
%         & VN & $ - \pm - $ & $- \pm -$ & $ - \pm - $ & $ - \pm - $ & \\
%         \cline{2-6}
%         & A-ConvMatch  & $ 58.72 \pm 0.40 $ & $ 61.70 \pm 0.53 $ & $ 63.61 \pm 0.35 $ & $ 66.52 \pm 0.59 $ & \\
%     \hline
%         \multirow{5}{*}{OGBNProducts} 
%         & RS & $ - \pm - $ & $- \pm -$ & $ - \pm - $ & $ - \pm - $ & \multirow{5}{*}{$ - \pm - $} \\
%         & KCenter & $ - \pm - $ & $- \pm -$ & $ - \pm - $ & $ - \pm - $ & \\
%         & Herding & $ - \pm - $ & $- \pm -$ & $ - \pm - $ & $ - \pm - $ & \\
%         & VN & $ - \pm - $ & $- \pm -$ & $ - \pm - $ & $ - \pm - $ & \\
%         \cline{2-6}
%         & A-ConvMatch  & $ - \pm - $ & $- \pm -$ & $ - \pm - $ & $ - \pm - $ & \\
%     \hline
%     \end{tabular}
%     \caption{Node Classification Accuracy at varying coarsening levels.}
%     \label{tab:my_label}
% \end{table*}
% }%

==> sections/tables/node_classification_graph_summarization_times.tex <==
{\small
\begin{table}[h]
    \centering
    \begin{tabular}{cc||ccc}
    \toprule
         & & \multicolumn{3}{c}{\textbf{Coarsening Ratio (r)}} \\
         \cline{3-5}
         & \textbf{Summarizer}  & $0.1\%$ & $1\%$ & $10\%$ \\
    \midrule
    \midrule
        \multirow{7}{*}{\rotatebox{90}{Citeseer}} 
        & KCenter & $ - $ & $ 179.33 \pm 1.70 $ & \cellcolor{orange!25} $ 179.55 \pm 1.77 $ \\
        & Herding & $ - $ & \cellcolor{orange!12} $ 177.17 \pm 1.93 $ & \cellcolor{orange!12} $ 179.56 \pm 3.74 $ \\
        & GCond & $ - $ & $ 940.25 \pm 2.51 $  & $ 3,879.38 \pm 4.36 $ \\
        & DosCond & $ - $ & \cellcolor{orange!25} $ 140.63 \pm 1.19 $ & $ 411.38 \pm 0.58 $ \\
        & VN & $ - $ & \cellcolor{orange!50} $ \mathbf{8.37 \pm 0.50} $ & \cellcolor{orange!50} $ \mathbf{8.05 \pm 0.58} $ \\
        \cline{2-5}
        & \shortname{}  & $ - $ & $ - \pm - $  & $ - \pm - $ \\
        & A-\shortname{}  & $ - $ & $ 203.93 \pm 3.29 $  & $ 190.94 \pm 3.35 $ \\
    \hline
    \hline
        \multirow{7}{*}{\rotatebox{90}{Cora}} 
        & KCenter & $ - $ & \cellcolor{orange!12} $ 160.60 \pm 2.53 $ & $ 159.97 \pm 2.76 $ \\
        & Herding & $ - $ & $ 162.71 \pm 3.01 $ & \cellcolor{orange!12} $ 159.61 \pm 2.19 $ \\
        & GCond & $ - $ & $ 1,179 \pm 32.47 $ &  $ 1,935 \pm 1.72 $ \\
        & DosCond & $ - $ & $ 250.64 \pm 8.02 $ &  $ 359.08 \pm 2.01 $ \\
        & VN & $ - $ & \cellcolor{orange!50} $ \mathbf{5.06 \pm 0.36} $ & \cellcolor{orange!50} $ \mathbf{5.12 \pm 0.42} $ \\
        \cline{2-5}
        & \shortname{}  & $ - $ & $ - \pm - $ &  $ - \pm - $ \\
        & A-\shortname{}  & $ - $ & \cellcolor{orange!25} $ 29.97 \pm 0.67 $ & \cellcolor{orange!25} $ 24.07 \pm 0.74 $ \\
    \hline
    \hline
        \multirow{6}{*}{\rotatebox{90}{OGBNArxiv}}
        & KCenter & $ 2,221 \pm 6.26 $ & $ 2,215 \pm 9.89 $ &  $ 2,292 \pm 23.85 $ \\
        & Herding & \cellcolor{orange!12} $ 2,214 \pm 13.25 $ & \cellcolor{orange!12} $ 2,210 \pm 9.81 $ & \cellcolor{orange!12} $ 2,242 \pm 6.52 $ \\
        & GCond & $ 14,475 \pm 373.65 $ & OOM & OOM \\
        & DosCond & $ 3,589 \pm 76.41 $ & OOM &  OOM \\
        & VN & \cellcolor{orange!25} $ 746.29 \pm 49.25 $ & \cellcolor{orange!25} $ 693.90 \pm 15.82 $ & \cellcolor{orange!25} $ 606.92 \pm 24.15 $ \\
        \cline{2-5}
        & A-\shortname{} & \cellcolor{orange!50} $ \mathbf{175.55 \pm 3.51} $ & \cellcolor{orange!50} $ \mathbf{148.80 \pm 2.54} $ & \cellcolor{orange!50} $ \mathbf{116.34 \pm 2.40} $ \\
    \hline
    \hline
        \multirow{6}{*}{\rotatebox{90}{OGBNProd}}
        & KCenter & $ - \pm - $ & $ - \pm - $ &  $ - $ \\
        & Herding & $ - \pm - $ & $ - \pm - $ &  $ - $ \\
        & GCond & OOM & OOM & $ - $ \\
        & DosCond & OOM & OOM &  $ - $ \\
        & VN & TIMEOUT & TIMEOUT &  $ - $ \\
        \cline{2-5}
        & A-\shortname{}  & \cellcolor{orange!50} $ \mathbf{8,090 \pm 14.66} $ & \cellcolor{orange!50} $ \mathbf{6,729 \pm 0.44} $ &  $ - $ \\
    \bottomrule
    \end{tabular}
    \caption{Node Classification Graph Summarization Times in Seconds at Varying Coarsening LevelsBest performing method is bolded. The top three performing scores are highlighted as: \colorbox{orange!50}{First}, \colorbox{orange!25}{Second}, \colorbox{orange!12}{Third}.}
    \label{tab:node_classification_summarization_time}
\end{table}
}%

% 0.001 0.01 0.1
% {\small
% \begin{table}[h]
%     \centering
%     \begin{tabular}{cc|ccc}
%     \toprule
%         & & \multicolumn{3}{c}{\textbf{Coarsening Ratio}} \\
%         \cline{3-5}
%         & \textbf{Summarizer}  & $\mathbf{r}=0.1\%$ & $\mathbf{r}=1\%$ & $\mathbf{r}=10\%$ \\
%     \midrule
%         \multirow{7}{*}{\rotatebox[origin=c]{90}{Citeseer}} 
%         & KCenter & $ 0.02 \pm 0.01 $ & $ 4.49 \pm 0.21 $ & $ 9.44 \pm 0.47 $ \\
%         & Herding & $ 0.03 \pm 0.00 $ & $ 3.39 \pm 0.09 $ & $ 6.62 \pm 0.55 $ \\
%         & GCond & $ 905 \pm 23.57 $ & $ 1,524 \pm 13.84 $ & $ 3,846 \pm 3.23 $ \\
%         & DosCond & $ 139 \pm 4.56 $ & $ 200 \pm 3.82 $ & $ 408 \pm 2.55 $ \\
%         & VN & $ 8.48 \pm 0.5 $ & $ 8.08 \pm 0.60 $ & $ 7.91 \pm 0.56 $ \\
%         \cline{2-5}
%         & \shortname{}  & $ - \pm - $ & $- \pm -$ & $ - \pm - $ \\
%         & A-\shortname{}  & $ 201 \pm 5.24 $ & $ 195 \pm 5.25 $ & $ 187 \pm 5.34 $ \\
%     \hline
%         \multirow{7}{*}{\rotatebox[origin=c]{90}{Cora}} 
%         & KCenter & $ 0.01 \pm 0.00 $ & $ 0.03 \pm 0.00 $ & $ 1.62 \pm 0.08 $ \\
%         & Herding & $ 0.02 \pm 0.00 $ & $ 0.04 \pm 0.01 $ & $ 0.32 \pm 0.01 $ \\
%         & GCond & $ 1,134 \pm - $ & $ 1,284 \pm -$ & OOM  \\
%         & DosCond & $ 247.11 \pm - $ & $ 265.58 \pm - $ & OOM \\
%         & VN & $ 5.25 \pm 0.56 $ & $ 4.60 \pm 0.04 $ & $ 5.36 \pm 0.47 $ \\
%         \cline{2-5}
%         & \shortname{}  & $ - \pm - $ & $ - \pm - $ & $ - \pm - $ \\
%         & A-\shortname{}  & $ 35.62 \pm 1.18 $ & $ 34.71 \pm 0.98 $ & $ 32.66 \pm 0.87 $ \\
%     \hline
%         \multirow{6}{*}{\rotatebox[origin=c]{90}{OGBNArxiv}} 
%         & KCenter & $ 5.60 \pm 0.18 $ & $ 41.22 \pm 2.05 $ & $ 124 \pm 1.14 $ \\
%         & Herding & $ 2.60 \pm 0.09 $ & $ 11.47 \pm 0.17 $ & $ 22.89 \pm 0.45 $ \\
%         & GCond & OOM & OOM & OOM \\
%         & DosCond & OOM & OOM & OOM \\
%         & VN & $ 701.93 \pm 20.95 $ & $ 669.60 \pm 23.80 $ & $ 611.79 \pm 31.33 $ \\
%         \cline{2-5}
%         & A-\shortname{}  & $ 309.94 \pm 28.6 $ & $ 266.81 \pm 25.00 $ & $ 245.48 \pm 21.76 $ \\
%     \hline
%         \multirow{4}{*}{\rotatebox[origin=c]{90}{OGBNProd}} 
%         & KCenter & $ - \pm - $ & $- \pm -$ & $ - \pm - $ \\
%         & Herding & $ - \pm - $ & $- \pm -$ & $ - \pm - $ \\
%         & VN & $ - \pm - $ & $- \pm -$ & $ - \pm - $ \\
%         \cline{2-5}
%         & A-\shortname{}  & $ - \pm - $ & $- \pm -$ & $ - \pm - $ \\
%     \bottomrule
%     \end{tabular}
%     \caption{Node Classification Graph Summarization Times in Seconds at Varying Coarsening Levels}
%     \label{tab:node_classification_summarization_time}
% \end{table}
% }%

% 0.01, 0.05, 0.1
% {\small
% \begin{table}[h]
%     \centering
%     \begin{tabular}{c|c|ccc}
%     \toprule
%         &  & $\mathbf{r}=0.01$ & $\mathbf{r}=0.05$ & $\mathbf{r}=0.1$ \\
%     \midrule
%         \multirow{7}{*}{\rotatebox[origin=c]{90}{Citeseer}} 
%         & KCenter & $ 0.02 \pm 0.01 $ & $ 4.49 \pm 0.21 $ & $ 9.44 \pm 0.47 $ \\
%         & Herding & $ 0.03 \pm 0.00 $ & $ 3.39 \pm 0.09 $ & $ 6.62 \pm 0.55 $ \\
%         & GCond & $ 905 \pm 23.57 $ & $ 1,524 \pm 13.84 $ & $ 3,846 \pm 3.23 $ \\
%         & DosCond & $ 139 \pm 4.56 $ & $ 200 \pm 3.82 $ & $ 408 \pm 2.55 $ \\
%         & VN & $ 8.48 \pm 0.5 $ & $ 8.08 \pm 0.60 $ & $ 7.91 \pm 0.56 $ \\
%         \cline{2-5}
%         & \shortname{}  & $ - \pm - $ & $- \pm -$ & $ - \pm - $ \\
%         & A-\shortname{}  & $ 201 \pm 5.24 $ & $ 195 \pm 5.25 $ & $ 187 \pm 5.34 $ \\
%     \hline
%         \multirow{7}{*}{\rotatebox[origin=c]{90}{Cora}} 
%         & KCenter & $ 0.01 \pm 0.00 $ & $ 0.03 \pm 0.00 $ & $ 1.62 \pm 0.08 $ \\
%         & Herding & $ 0.02 \pm 0.00 $ & $ 0.04 \pm 0.01 $ & $ 0.32 \pm 0.01 $ \\
%         & GCond & $ 1,134 \pm - $ & $ 1,284 \pm -$ & OOM  \\
%         & DosCond & $ 247.11 \pm - $ & $ 265.58 \pm - $ & OOM \\
%         & VN & $ 5.25 \pm 0.56 $ & $ 4.60 \pm 0.04 $ & $ 5.36 \pm 0.47 $ \\
%         \cline{2-5}
%         & \shortname{}  & $ - \pm - $ & $ - \pm - $ & $ - \pm - $ \\
%         & A-\shortname{}  & $ 35.62 \pm 1.18 $ & $ 34.71 \pm 0.98 $ & $ 32.66 \pm 0.87 $ \\
%     \hline
%         \multirow{6}{*}{\rotatebox[origin=c]{90}{OGBNArxiv}} 
%         & KCenter & $ 5.60 \pm 0.18 $ & $ 41.22 \pm 2.05 $ & $ 124 \pm 1.14 $ \\
%         & Herding & $ 2.60 \pm 0.09 $ & $ 11.47 \pm 0.17 $ & $ 22.89 \pm 0.45 $ \\
%         & GCond & OOM & OOM & OOM \\
%         & DosCond & OOM & OOM & OOM \\
%         & VN & $ 701.93 \pm 20.95 $ & $ 669.60 \pm 23.80 $ & $ 611.79 \pm 31.33 $ \\
%         \cline{2-5}
%         & A-\shortname{}  & $ 309.94 \pm 28.6 $ & $ 266.81 \pm 25.00 $ & $ 245.48 \pm 21.76 $ \\
%     \hline
%         \multirow{4}{*}{\rotatebox[origin=c]{90}{OGBNProd}} 
%         & KCenter & $ - \pm - $ & $- \pm -$ & $ - \pm - $ \\
%         & Herding & $ - \pm - $ & $- \pm -$ & $ - \pm - $ \\
%         & VN & $ - \pm - $ & $- \pm -$ & $ - \pm - $ \\
%         \cline{2-5}
%         & A-\shortname{}  & $ - \pm - $ & $- \pm -$ & $ - \pm - $ \\
%     \bottomrule
%     \end{tabular}
%     \caption{Node Classification Graph Summarization Times in Seconds at Varying Coarsening Levels}
%     \label{tab:node_classification_summarization_time}
% \end{table}
% }%

% With 0.3
% {\small
% \begin{table*}[h]
%     \centering
%     \begin{tabular}{cc|cccc}
%     \hline
%         \textbf{Dataset} & \textbf{Summarizer} & $\mathbf{r}=0.01$ & $\mathbf{r}=0.05$ & $\mathbf{r}=0.1$ & $\mathbf{r}=0.3$\\
%     \midrule
%         \multirow{5}{*}{Citeseer} 
%         & KCenter & $ 0.02 \pm 0.01 $ & $ 4.49 \pm 0.21 $ & $ 9.44 \pm 0.47 $ & $ 35.64 \pm 0.48 $ \\
%         & Herding & $ 0.03 \pm 0.00 $ & $ 3.39 \pm 0.09 $ & $ 6.62 \pm 0.55 $ & $ 17.45 \pm 1.47 $ \\
%         & GCond & $ 905 \pm 23.57 $ & $ 1,524 \pm 13.84 $ & $ 3,846 \pm 3.23 $ & $ - \pm - $ \\
%         & DosCond & $ 139 \pm 4.56 $ & $ 200 \pm 3.82 $ & $ 408 \pm 2.55 $ & $ - \pm - $ \\
%         & VN & $ 8.48 \pm 0.5 $ & $ 8.08 \pm 0.60 $ & $ 7.91 \pm 0.56 $ & $ 7.99 \pm 0.47 $ \\
%         \cline{2-6}
%         & \shortname{}  & $ - \pm - $ & $- \pm -$ & $ - \pm - $ & $ - \pm - $ \\
%         & A-\shortname{}  & $ 201 \pm 5.24 $ & $ 195 \pm 5.25 $ & $ 187 \pm 5.34 $ & $ 155 \pm 5.41 $ \\
%     \hline
%         \multirow{5}{*}{Cora} 
%         & KCenter & $ 0.01 \pm 0.00 $ & $ 0.03 \pm 0.00 $ & $ 1.62 \pm 0.08 $ & $ 4.61 \pm 0.16 $ \\
%         & Herding & $ 0.02 \pm 0.00 $ & $ 0.04 \pm 0.01 $ & $ 0.32 \pm 0.01 $ & $ 0.88 \pm 0.03 $ \\
%         & GCond & $ 1,134 \pm - $ & $ 1,284 \pm -$ & OOM & OOM \\
%         & DosCond & $ 247.11 \pm - $ & $ 265.58 \pm - $ & OOM & OOM \\
%         & VN & $ 5.25 \pm 0.56 $ & $ 4.60 \pm 0.04 $ & $ 5.36 \pm 0.47 $ & $ 4.85 \pm 0.52 $ \\
%         \cline{2-6}
%         & \shortname{}  & $ - \pm - $ & $ - \pm - $ & $ - \pm - $ & $ - \pm - $ \\
%         & A-\shortname{}  & $ 35.62 \pm 1.18 $ & $ 34.71 \pm 0.98 $ & $ 32.66 \pm 0.87 $ & $ 25.93 \pm 0.75 $ \\
%     \hline
%         \multirow{5}{*}{OGBNArxiv} 
%         & KCenter & $ 5.60 \pm 0.18 $ & $ 41.22 \pm 2.05 $ & $ 124 \pm 1.14 $ & $ 887 \pm 14.8 $ \\
%         & Herding & $ 2.60 \pm 0.09 $ & $ 11.47 \pm 0.17 $ & $ 22.89 \pm 0.45 $ & $ 70.53 \pm 1.20 $ \\
%         & GCond & OOM & OOM & OOM & OOM \\
%         & DosCond & OOM & OOM & OOM & OOM \\
%         & VN & $ 701.93 \pm 20.95 $ & $ 669.60 \pm 23.80 $ & $ 611.79 \pm 31.33 $ & $ 579.80 \pm 14.67 $ \\
%         \cline{2-6}
%         & A-\shortname{}  & $ 309.94 \pm 28.6 $ & $ 266.81 \pm 25.00 $ & $ 245.48 \pm 21.76 $ & $ 189.97 \pm 17.48 $ \\
%     \hline
%         \multirow{5}{*}{OGBNProducts} 
%         & KCenter & $ - \pm - $ & $- \pm -$ & $ - \pm - $ & $ - \pm - $ \\
%         & Herding & $ - \pm - $ & $- \pm -$ & $ - \pm - $ & $ - \pm - $ \\
%         & VN & $ - \pm - $ & $- \pm -$ & $ - \pm - $ & $ - \pm - $ \\
%         \cline{2-6}
%         & A-\shortname{}  & $ - \pm - $ & $- \pm -$ & $ - \pm - $ & $ - \pm - $ \\
%     \hline
%     \end{tabular}
%     \caption{Node Classification Graph Summarization Times in Seconds at Varying Coarsening Levels}
%     \label{tab:my_label}
% \end{table*}
% }%

==> sections/tables/node_classification_training_times.tex <==
{\small
\begin{table}[h]
    \centering
    \begin{tabular}{cc||cccc}
    \toprule
         & & \multicolumn{4}{c}{\textbf{Coarsening Ratio (r)}} \\
         \cline{3-6}
         & \textbf{Summarizer}  & $0.1\%$ & $1\%$ & $10\%$ & $100\%$ \\
    \midrule
    \midrule
        \multirow{7}{*}{\rotatebox{90}{Citeseer}}
        & KCenter & $ - $ & $ - \pm - $ &  $ - \pm - $ & \multirow{7}{*}{\rotatebox{90}{$ \mathbf{ 314.71 \pm 2.89 }$}} \\
        & Herding & $ - $ & $ - \pm - $ &  $ - \pm - $ & \\
        & GCond & $ - $ & $ 160.94 \pm 18.14 $ &  $ 177.42 \pm 4.91 $ & \\
        & DosCond & $ - $ & $ 153.58 \pm 2.51 $ &  $ 179.02 \pm 4.60 $ & \\
        & VN & $ - $ & $ 130.13 \pm 2.91 $ &  $ 151.40 \pm 1.86 $ & \\
        \cline{2-5}
        & \shortname{}  & $ - $ & $ - \pm - $ &  $ - \pm - $ & \\
        & A-\shortname{}  & $ - $ & $ 249.55 \pm 8.34 $ &  $ 313.08 \pm 2.06 $ & \\
    \hline
    \hline
        \multirow{7}{*}{\rotatebox{90}{Cora}} 
        & KCenter & $ - $ & $ 235.91 \pm 1.83 $ &  $ 236.08 \pm 0.15 $ & \multirow{7}{*}{\rotatebox{90}{$\mathbf{ 579.81 \pm 10.03 }$}} \\
        & Herding & $ - $ & $ 238.54 \pm 1.24 $ &  $ 233.86 \pm 0.94 $ & \\
        & GCond & $ - $ & $ 306.32 \pm 4.46 $ &  $ 331.78 \pm 1.13 $ & \\
        & DosCond & $ - $ & $ 304.45 \pm 2.98 $ &  $ 326.28 \pm 5.13 $ & \\
        & VN & $ - $ & $ 271.28 \pm 12.38 $ &  $ 307.16 \pm 3.88 $ & \\
        \cline{2-5}
        & \shortname{}  & $ - $ & $ - \pm - $ &  $ - \pm - $ & \\
        & A-\shortname{}  & $ - $ & $ 248.55 \pm 2.48 $ &  $ 562.94 \pm 2.09 $ & \\
    \hline
    \hline
        \multirow{6}{*}{\rotatebox{90}{OGBNArxiv}}
        & KCenter & $ - \pm - $ & $ - \pm - $ &  $ - \pm - $ & \multirow{6}{*}{\rotatebox{90}{$ \mathbf{ 4,508.86 \pm 54.52 }$}} \\
        & Herding & $ - \pm - $ & $ - \pm - $ &  $ - \pm - $ & \\
        & GCond & $ - \pm - $ & OOM &  OOM & \\
        & DosCond & $ - \pm - $ & OOM &  OOM & \\
        & VN & $ 154.00 \pm 2.18 $ & $ 172.78 \pm 2.60 $ &  $ 213.56 \pm 5.22 $ & \\
        \cline{2-5}
        & A-\shortname{}  & $ 168.90 \pm 0.64 $ & $ 335.89 \pm 3.29 $ &  $ 738.07 \pm 5.77 $ & \\
    \hline
    \hline
        \multirow{6}{*}{\rotatebox{90}{OGBNProd}}
        & KCenter & $ - \pm - $ & $ - \pm - $ &  $ - \pm - $ & \multirow{6}{*}{\rotatebox{90}{$ \mathbf{ - \pm - }$}} \\
        & Herding & $ - \pm - $ & $ - \pm - $ &  $ - \pm - $ & \\
        & GCond & $ - \pm - $ & $ - \pm - $ &  $ - \pm - $ & \\
        & DosCond & $ - \pm - $ & $ - \pm - $ &  $ - \pm - $ & \\
        & VN & $ - \pm - $ & $ - \pm - $ &  $ - \pm - $ & \\
        \cline{2-5}
        & A-\shortname{}  & $ - \pm - $ & $ - \pm - $ &  $ - \pm - $ & \\
    \bottomrule
    \end{tabular}
    \caption{Node Classification Training Times at Varying Coarsening Levels}
    \label{tab:node_classification_training_time}
\end{table}
}%

% {\small
% \begin{table*}[h]
%     \centering
%     \begin{tabular}{cc|cccc}
%     \hline
%         \textbf{Dataset} & \textbf{Graph Summarizer} & $\mathbf{r}=0.01$ & $\mathbf{r}=0.1$ & $\mathbf{r}=0.3$ & $\mathbf{r}=0.5$ \\
%     \midrule
%         \multirow{6}{*}{Citeseer} 
%         & Random Node Sampler & $- \pm -$ & $- \pm -$ & $- \pm -$ & \multirow{6}{*}{$54 \pm 2$}  \\
%         & Herding & $ 49 \pm 1 $ & $ 50 \pm 2 $ & $ 52 \pm 0 $ & \\
%         & KCenter & $ 48 \pm 1 $ & $ 48 \pm 1 $ & $ 52 \pm 2 $ & \\
%         & Variation Neighborhoods & $ 51 \pm 3 $ & $ 53 \pm 2 $ & $ 52 \pm 1 $ & \\\cline{2-5}
%         & Conv. Matching & $- \pm -$ & $- \pm -$ & $- \pm -$ & \\
%         & Approx. Conv. Matching & $ 46 \pm 2 $ & $ 53 \pm 1.2 $ & $ 53 \pm 0 $ & \\
%     \hline
%         \multirow{6}{*}{Cora} 
%         & Random Node Sampler & $- \pm -$ & $- \pm -$ & $- \pm -$ & \multirow{6}{*}{$ 52 \pm 0 $} \\
%         & Herding & $ 46 \pm 0 $ & $ 46 \pm 0 $ & $ 50 \pm 0 $ & \\
%         & KCenter & $ 47 \pm 1 $ & $ 46 \pm 2 $ & $ 48 \pm 1 $ & \\
%         & Variation Neighborhoods & $ 49 \pm 1 $ & $ 51 \pm 1 $ & $ 51 \pm 1 $ & \\\cline{2-5}
%         & Conv. Matching & $- \pm -$ & $- \pm -$ & $- \pm -$ & \\
%         & Approx. Conv. Matching & $ 45 \pm 3 $ & $ 51 \pm 1 $ & $ 52 \pm 1 $ & \\
%     \hline
%         \multirow{5}{*}{OGBNArxiv} 
%         & Random Node Sampler & $ 762 \pm 14 $ & $ 839 \pm 17 $ & $ 974 \pm 10 $ & \multirow{5}{*}{$ 2,122 \pm 23 $}  \\
%         & Herding & $ 764 \pm 8 $ & $ 893 \pm 15 $ & $ 1,152 \pm 16 $ & \\
%         & KCenter & $ 766 \pm 8 $ & $ 894 \pm 13 $ & $ 1,144 \pm 21 $ & \\
%         & Variation Neighborhoods & $ 778 \pm 13 $ & $ 770 \pm 9 $ & $ 1,081 \pm 15 $ &  \\\cline{2-5}
%         & Approx. Conv. Matching & $ 775 \pm 4 $ & $ 937 \pm 8 $ & $ 1,202 \pm 15 $ & \\
%     \hline
%         \multirow{5}{*}{OGBNProducts} 
%         & Random Node Sampler & $- \pm -$ & $- \pm -$ & $- \pm -$ & $- \pm -$  \\
%         & Herding & $- \pm -$ & $- \pm -$ & $- \pm -$ & $- \pm -$  \\
%         & KCenter & $- \pm -$ & $- \pm -$ & $- \pm -$ & $- \pm -$  \\
%         & Variation Neighborhoods & $- \pm -$ & $- \pm -$ & $- \pm -$ & $- \pm -$  \\\cline{2-6}
%         & Approx. Conv. Matching & $- \pm -$ & $- \pm -$ & $- \pm -$ & $- \pm -$ \\
%     \hline
%     \end{tabular}
%     \caption{Node Classification Training Times in Seconds at Varying Coarsening Levels}
%     \label{tab:my_label}
% \end{table*}
% }%
